NSBchain: A Secure Blockchain Framework for Network Slicing Brokerage

With the advent of revolutionary technologies, such as virtualization and softwarization, a novel concept for 5G networks and beyond has been unveiled: Network Slicing. Initially driven by the research community, standardization bodies as 3GPP have embraced it as a promising solution to revolutionize the traditional mobile telecommunication market by enabling new business models opportunities. Network Slicing is envisioned to open up the telecom market to new players such as Industry Verticals, e.g. automotive, smart factories, e-health, etc. Given the large number of potential new business players, dubbed as network tenants, novel solutions are required to accommodate their needs in a cost-efficient and secure manner. In this paper, we propose NSBchain, a novel network slicing brokering (NSB) solution, which leverages on the widely adopted Blockchain technology to address the new business models needs beyond traditional network sharing agreements. NSBchain defines a new entity, the Intermediate Broker (IB), which enables Infrastructure Providers (InPs) to allocate network resources to IBs through smart contracts and IBs to assign and re-distribute their resources among tenants in a secure, automated and scalable manner. We conducted an extensive performance evaluation by means of an open-source blockchain platform that proves the feasibility of our proposed framework considering a large number of tenants and two different consensus algorithms.

==> perfeval.tex <==
\section{Proof-of-Concept Evaluation}
\label{sec:perf_eval}
We implement \name{} on top of Hyperledger Fabric~\cite{HyperledgerFabric}, an open-source framework for developing permissioned blockchains within private enterprises, and make use of its benchmarking tool, namely Hyperledger Caliper, to evaluate the blockchain performance in network slicing scenarios. 

\indent \textbf{Experimental setup.} Our Proof-of-Concept (PoC) architecture consists of $3$ IBs and a variable number of orderer nodes that depends on the adopted consensus algorithm. Such entities run as Docker containers on an Intel Xeon CPU E5-2630v3 32-Core @2.4GHz 64GB RAM shared platform. %While such a deployment cannot evaluate performances in an enterprise-grade deployment as per~\cite{Performance_Benchmarking}, it suggests the applicability of our solution within realistic network slice brokering scenarios.
%Indeed, we do not aim at measuring peak performances in an enterprise-grade deployment, as e.g. shown in~\cite{Performance_Benchmarking}, but rather study the applicability of our solution at the network slice brokering scenario.

\begin{figure*}[t!]
    \centering
    	  \begin{subfigure}[b]{.48\textwidth}
          \includegraphics[trim = 0cm 0cm 0cm 0cm,clip, width=\linewidth]{figs/barplot.pdf}
          \caption{Slice request throughput and blockchain size growth for \\ different consensus algorithms and consortium size. }
          \label{fig:transaction_throughput}
      \end{subfigure}%
	  \begin{subfigure}[b]{.49\textwidth}
          \includegraphics[trim = 0cm 0cm 0cm 0cm,clip, width=\linewidth]{figs/latency.pdf}
        \caption{CDF of the slice request validation latency experienced by tenants for different consensus algorithms and consortium size.}
        \label{fig:transaction_latency}
      \end{subfigure}%
    \caption{\small Performance evaluation for different consensus algorithms and consortium size a) Slice request throughput and Blockchain size growth b) Validation latency.}
	\label{fig:sims_results}
\vspace{-4mm}
\end{figure*}


We guarantee the isolation among consortia through the definition of dedicated and encrypted communication channels. Moreover, we set the maximum number of entries per block to $20$ and the block timeout\footnote{We select such values as they maximize the throughput at a minimum latency cost as proved hereafter in the section.} to $300$ ms.
This last metric specifies the amount of time (after receiving the first transaction) each orderer waits before publishing a new set of proposed transactions to other peer nodes.
%
Please note that the choice of those parameters may strongly affect the blockchain performance. In particular, although decreasing the block timeout improves the latency, setting it with low values may decrease the overall throughput as new blocks would not be filled up to their maximum capacity. To limit the impact of this trade-off on our results, we do not modify these settings throughout this section. 

The benchmark process consists of two phases, dubbed as opening and transfer. In the initial phase, we create tenant instances and assign them with an equal amount of resources such that all available resources at IB side are assigned. Once assigned, each tenant might decide to free or seek additional resources based on a random value drawn from a uniform distribution between $0$ and $30\%$ of the initially assigned amount\footnote{We empirically prove that the choice of this value leads to convergence within a reasonable time.}. During the transfer phase, tenants issue Slice Requests (SRs), modeled as tuples $\Psi_\tau = \{\rho, \eta, \gamma \}$, where $\rho, \eta, \gamma \in \mathcal{R}_k$ represent the percentage of required radio access, transport and core cloud resources, respectively. In case the SR does not fit the availability or the need of the involved tenants (SR collision), it is automatically rejected and the respective transaction is dropped.

\indent \textbf{Full-scale evaluation.} With the first experiment we evaluate the performance of our framework in terms of slice request throughput and latency. We compare two popular consensus algorithms (Kafka and Raft) against a single orderer configuration (Solo) that does not require any consensus process. The top of Fig.~\ref{fig:transaction_throughput} shows the average SR throughput of the platform in the transfer phase for an increasing consortium size and fixed SR rate of $150$ SRs/s to emulate high load conditions. In these settings, especially for a small consortium size, the limiting factor of the blockchain performance throughput is the Multiversion Concurrency Control (MVCC) process. As we issue SRs at a very high rate, the same database entry, e.g. the resources assigned to a specific tenant, may be edited by a new request before the completion of the validation process involving it.
This raises a database inconsistency, dubbed as Read/Write (RW) conflict, which prevents the current transaction to be successful. As shown in the figure, this problem is mitigated by an increasing consortium size.

%the average transaction throughput handled by the platform increases with the consortium size 
%since the bigger the consortium the lower is the probability that two transactions in the same block target the same database key.
Fig.~\ref{fig:transaction_latency} depicts the Cumulative Distribution Function (CDF) of the experienced latency by the successful SRs.
As expected, the best latency performance is obtained when no distributed consensus mechanism is in place, i.e., Solo. However, despite being the fastest scheme, this single-node approach is not fault tolerant.
It can be noticed that the transaction exchange and validation process introduce a small time overhead for the Kafka and Raft cases, which however has negligible impact, especially when compared to the onboarding time required e.g., by virtualized infrastructures to setup virtual services~\cite{BSecNFVO}.
The blockchain growth rate is also affected by the different consensus scheme, as shown at the bottom of Fig.~\ref{fig:transaction_throughput}, which refers to the consortium size case of $1000$ tenants. We plot the evolution of the chain size over time and mark the beginning of the transfer phase with a dashed vertical line. It can be noticed that the blockchain grows at a rate proportional to the average throughput since blocks are filled up to their maximum capacity.

%Moreover, the higher throughput provided by Kafka is often achieved at the cost of some additional latency with respect to Raft. \\
\indent \textbf{Brokering scenario evaluation.}
The second experiment focuses on evaluating the capabilities of the system when dealing with the brokering scenario. To this aim, we consider $3$ IBs managing a consortium of $1000$ tenants, correspondingly. In light of the performances shown above, we select Kafka as consensus algorithm for its high fault-tolerance and scalability~\cite{Performance_Benchmarking}. We assume that resource request values $\rho, \eta, \gamma$ are drawn from a right-skewed distribution over a positive interval as resource requests must be non-negative. Such distributions are depicted at the top of Fig.~\ref{fig:acceptance_rate} for different demand ranges, spanning from $0.1$\% to $4$\% of the tenant initial resources. Note that since we assume the same distribution for all resource requests within the same slice, it is dubbed as SR PDF.

The bottom of Fig.~\ref{fig:acceptance_rate} illustrates the system behavior for a constant submission rate of $50$ SRs/s so as to keep RW Conflicts to a minimum (around $2\%$ of the submitted SRs). In such operational conditions, errors raise only in case of SR collisions. It is worth noting that SR collision rate increases along with the SR variance. Specifically, SR distributions with high variance leads to tenant satisfaction more quickly than with a lower variance. Additionally, the closer to tenant satisfaction, the lower the resource availability and, in turn, the smaller the likelihood of a request to be accepted by the system.
\begin{figure}[t!]
      \centering
      \includegraphics[clip, trim= 0cm 0cm 0cm 0cm,   width=0.48\textwidth]{figs/acceptance_rate.pdf}
      \caption{\small Transaction acceptance and error rates for different scenarios.}
        \label{fig:acceptance_rate}
\end{figure}
